Best-first Search Algorithm for Non-convex Sparse Minimization

Non-convex sparse minimization (NSM), or $\ell_0$-constrained minimization of convex loss functions, is an important optimization problem that has many machine learning applications. NSM is generally NP-hard, and so to exactly solve NSM is almost impossible in polynomial time. As regards the case of quadratic objective functions, exact algorithms based on quadratic mixed-integer programming (MIP) have been studied, but no existing exact methods can handle more general objective functions including Huber and logistic losses; this is unfortunate since those functions are prevalent in practice. In this paper, we consider NSM with $\ell_2$-regularized convex objective functions and develop an algorithm by leveraging the efficiency of best-first search (BFS). Our BFS can compute solutions with objective errors at most $\Delta\ge0$, where $\Delta$ is a controllable hyper-parameter that balances the trade-off between the guarantee of objective errors and computation cost. Experiments demonstrate that our BFS is useful for solving moderate-size NSM instances with non-quadratic objectives and that BFS is also faster than the MIP-based method when applied to quadratic objectives.

==> tex/package_back.tex <==
\usepackage{amsmath,amssymb}
%\usepackage[dvipdfmx]{graphicx}
\usepackage{latexsym}
\usepackage{bm}
\usepackage{setspace}
\usepackage{enumerate}
%\usepackage{listings, jlisting}
\usepackage{amsthm}
\usepackage{cases}
\usepackage{mathrsfs}
\usepackage{mathtools}
%\usepackage{subcaption}
\usepackage{comment}
\usepackage{url}
\usepackage{array}

\usepackage{wrapfig}
\usepackage{tikz}
\usepackage{tikz-3dplot}
\usetikzlibrary{positioning}

%\usepackage{algorithm, algorithmic}

\usepackage{multirow}
%\usepackage{color}

\mathtoolsset{showonlyrefs=true}



%\usepackage{algorithmic, algorithmicx}
%\usepackage[noend]{algorithm, algpseudocode}
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}

==> tex/settings.tex <==
\lstset{
    language=Matlab,%プログラミング言語によって変える。
    basicstyle={\ttfamily\small},
    tabsize=2,
    frame=trBL,
    numbers=left,
    numberstyle={\ttfamily\small},
    breaklines=true,%折り返し
    captionpos=b
}
\makeatletter
    \renewcommand{\theequation}{%
    \thesection.\arabic{equation}}
    \@addtoreset{equation}{section}
\makeatother

\topmargin = -10pt
\oddsidemargin = -10pt
\evensidemargin = -10pt
\headheight = -8pt
\textheight = 638pt
\textwidth = 445pt

\setstretch{1.05}

